Visual Prompting for Generalized Few-shot Segmentation: A Multi-scale Approach

The emergence of attention-based transformer models has led to their extensive use in various tasks, due to their superior generalization and transfer properties. Recent research has demonstrated that such models, when prompted appropriately, are excellent for few-shot inference. However, such techniques are under-explored for dense prediction tasks like semantic segmentation. In this work, we examine the effectiveness of prompting a transformer-decoder with learned visual prompts for the generalized few-shot segmentation (GFSS) task. Our goal is to achieve strong performance not only on novel categories with limited examples, but also to retain performance on base categories. We propose an approach to learn visual prompts with limited examples. These learned visual prompts are used to prompt a multiscale transformer decoder to facilitate accurate dense predictions. Additionally, we introduce a unidirectional causal attention mechanism between the novel prompts, learned with limited examples, and the base prompts, learned with abundant data. This mechanism enriches the novel prompts without deteriorating the base class performance. Overall, this form of prompting helps us achieve state-of-the-art performance for GFSS on two different benchmark datasets: COCO-$20^i$ and Pascal-$5^i$, without the need for test-time optimization (or transduction). Furthermore, test-time optimization leveraging unlabelled test data can be used to improve the prompts, which we refer to as transductive prompt tuning.

==> sec/conclusion_original.tex <==


\vspace{-4pt}
In this work, we proposed a technique to learn visual prompts from few-shot examples of novel unseen cateogries to prompt a pre-trained segmentation model that not only generalizes well on the unseen novel class but strongly retains performance over the base classes on which the model was pre-trained. We achieve this by prompting the image features at multiple-scales and proposing a uni-directional novel-to-base causal attention mechanism that enriches the features novel visual prompts through interaction with the base visual prompts. Our proposed method can be applied in both inductive and transductive settings and achieves state-of-the-art performance on two benchmark few-shot segmentation datasets.

==> sec/experiments_original.tex <==
\label{sec:exps}

\begin{table*}[t!]
\centering

 \begin{adjustbox}{max width=0.70\textwidth}
\begin{tabu}{@{}llcccccc@{}}
\tabucline[1pt]{-}
\multirow{1}{*}{} & \multirow{1}{*}{} & \multicolumn{6}{c}{} \\ 
 &  &  \multicolumn{6}{c}{\textbf{COCO-$20^i$}}\\

\multirow{2}{*}{Method} & \multirow{2}{*}{Learning} & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{5-shot}\\ 

\cmidrule(r{2pt}){3-5} \cmidrule(r{2pt}){6-8}

 & & Base  & Novel & Mean & Base & Novel & Mean  \\ \hline
% CANeT~\cite{tian2022generalized} \ \tt{(CVPR '22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\
% PANET~\cite{tian2022generalized} \ \tt{(CVPR '22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\
% PFENET~\cite{tian2022generalized} \ \tt{(CVPR '22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\
% MiB~\cite{tian2022generalized} \ \tt{(CVPR '22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\
% SCL~\cite{tian2022generalized} \ \tt{(CVPR '22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\
CAPL~\cite{tian2022generalized} \ \tt{(CVPR22)}  & Inductive & 43.21 & 7.21 & 25.21 &  43.71 & 11.00 & 27.36\\

BAM~\cite{lang2022learning} \ \tt{(CVPR22)}  & Inductive & 49.84 & 14.16 & 32.00 &  49.85 & 16.63 & 33.24\\

DIaM (w/o trans.)$^*$ ~\cite{hajimiri2023strong}   \ \tt{(CVPR23)}  & Inductive & 42.69 & 15.32 & 29.00 &  38.47 & 20.87 & 29.67\\
POP$^\dagger$~\cite{liu2023learning} \ \tt{(CVPR23)}  & Inductive & 30.38 & 9.63 & 20.00 &  24.53 & 16.19 & 20.36\\
\textbf{Ours (w/o trans.)} & Inductive & \textbf{51.55} & \textbf{18.00} & \textbf{34.78} &  \textbf{51.59} & \textbf{30.06} & \textbf{40.83}\\

\hline
RePRI~\cite{boudiaf2021few} \ \tt{(CVPR21)}  & Transductive & 5.62 & 4.74 & 5.18 &  8.85 & 8.84 & 8.85\\

DIaM~\cite{hajimiri2023strong} \tt{(CVPR23)}  & Transductive & 48.28 & 17.22 & 32.75 &  48.37 & 28.73 & 38.55\\

POP$^\dagger$~\cite{liu2023learning} \ \tt{(CVPR23)}  & Transductive & \textbf{54.71} & 15.31 & 35.01 &  \textbf{54.90} & 29.97 & 42.44\\

\textbf{Ours (w/ trans.) }& Transductive & \underline{53.80} & \textbf{18.30} & \textbf{36.05} & \underline{53.81} & \textbf{31.14} & \textbf{42.48}\\

\tabucline[1pt]{-}
\multirow{1}{*}{} & \multirow{1}{*}{} & \multicolumn{6}{c}{} \\ 
\multirow{1}{*}{} & \multirow{1}{*}{} & \multicolumn{6}{c}{\textbf{PASCAL-$5^i$}} \\ 
\multirow{2}{*}{Method} & \multirow{2}{*}{Learning} & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{5-shot}  \\ 

\cmidrule(r{2pt}){3-5} \cmidrule(r{2pt}){6-8}

 & & Base  & Novel & Mean & Base & Novel & Mean  \\ \hline
CANeT~\cite{zhang2019canet} \ \tt{(CVPR19)}  & Inductive & 8.73 & 2.42 & 5.58 &  9.05 & 1.52 & 5.29\\
PFENET~\cite{tian2020prior} \ \tt{(TPAMI20)}  & Inductive & 8.32 & 2.67 & 5.50 &  8.83 & 1.89 & 5.36\\
PANET~\cite{wang2019panet} \ \tt{(ICCV19)}  & Inductive & 31.88 & 11.25 & 21.57 &  32.95 & 15.25 & 24.1\\

SCL~\cite{zhang2021self} \ \tt{(CVPR21)}  & Inductive & 8.88 & 2.44 & 5.66 &  9.11 & 1.83 & 5.47\\

MiB~\cite{cermelli2020modeling} \ \tt{(CVPR20)}  & Inductive & 63.80 & 8.86 & 36.33 &  68.60 & 28.93 & 48.77\\

CAPL~\cite{tian2022generalized} \ \tt{(CVPR22)}  & Inductive & 64.80 & 17.46 & 41.13 &  65.43 & 24.43 & 44.93\\

BAM~\cite{lang2022learning} \ \tt{(CVPR22)}  & Inductive & 71.60 & 27.49 & 49.55 &  71.60 & 28.96 & 50.28\\

DIaM (w/o trans.)$^*$ ~\cite{hajimiri2023strong}  \tt{(CVPR23)} & Inductive  & 66.79 & 27.36 & 47.08 & 64.05 & 34.56 & 49.31\\

POP$^\dagger$~\cite{liu2023learning} \ \tt{(CVPR23)}  & Inductive & 46.68 & 19.96 & 33.32 &  41.50 & 36.26 & 38.80\\

\textbf{Ours (w/o trans.)} & Inductive & \textbf{74.58} & \textbf{34.99} & \textbf{54.79} &  \textbf{74.86} & \textbf{50.34} & \textbf{62.60}\\

\hline
RePRI~\cite{boudiaf2021few} \ \tt{(CVPR21)}  & Transductive & 20.76 & 10.50 & 15.63 &  34.06 & 20.98 & 27.52\\

DIaM~\cite{hajimiri2023strong} \tt{(CVPR23)} & Transductive & 70.89 & 35.11 & 53.00 &  70.85  & 55.31 & 63.08\\

POP$^\dagger$~\cite{liu2023learning} \ \tt{(CVPR23)}  & Transductive & 73.92 & 35.51 & 54.72 &  74.78 & 55.87 & 65.33\\

\textbf{Ours (w/ trans.) }& Transductive & \textbf{76.39} & \textbf{39.83} & \textbf{58.11} &  \textbf{76.42} & \textbf{56.12} & \textbf{66.27}\\

\tabucline[1pt]{-}

\end{tabu}
\end{adjustbox}
\captionsetup{labelfont=bf}
\captionof{table}{{\bf Comparison to SoTA methods on COCO-$20^i$ and PASCAL-$5^i$.} The mIoU results are reported as the average across 5 different runs. All methods use ResNet-50 backbone. Results of the previous methods obtained from ~\cite{hajimiri2023strong} except the inductive setting of DIaM (marked with $^*$), the results of which we obtained ourselves. The \textbf{w/o trans.},\textbf{ w/ trans.} denote without and with transduction respectively. }
\vspace{-0.1in}
 \label{tab:coco}
\end{table*}


% \begin{table*}[t!] 
% \centering
%  \begin{adjustbox}{max width=0.7\textwidth}
% \begin{tabu}{@{}llcccccc@{}}
% \tabucline[1pt]{-}
% \multirow{2}{*}{Method} & \multirow{2}{*}{Learning Type} & \multicolumn{3}{c}{1-shot} & \multicolumn{3}{c}{5-shot}\\ 

% \cmidrule(r{2pt}){3-5} \cmidrule(r{2pt}){6-8}

%  & & Base  & Novel & Mean & Base & Novel & Mean  \\ \hline
% CANeT~\cite{zhang2019canet} \ \tt{(CVPR19)}  & Inductive & 8.73 & 2.42 & 5.58 &  9.05 & 1.52 & 5.29\\
% PFENET~\cite{tian2020prior} \ \tt{(TPAMI20)}  & Inductive & 8.32 & 2.67 & 5.50 &  8.83 & 1.89 & 5.36\\
% PANET~\cite{wang2019panet} \ \tt{(ICCV19)}  & Inductive & 31.88 & 11.25 & 21.57 &  32.95 & 15.25 & 24.1\\

% SCL~\cite{zhang2021self} \ \tt{(CVPR21)}  & Inductive & 8.88 & 2.44 & 5.66 &  9.11 & 1.83 & 5.47\\

% MiB~\cite{cermelli2020modeling} \ \tt{(CVPR20)}  & Inductive & 63.80 & 8.86 & 36.33 &  68.60 & 28.93 & 48.77\\

% CAPL~\cite{tian2022generalized} \ \tt{(CVPR22)}  & Inductive & 64.80 & 17.46 & 41.13 &  65.43 & 24.43 & 44.93\\

% BAM~\cite{lang2022learning} \ \tt{(CVPR22)}  & Inductive & 71.60 & 27.49 & 49.55 &  71.60 & 28.96 & 50.28\\

% DIaM (w/o trans.)~\cite{hajimiri2023strong}  \tt{(CVPR23)} & Inductive  & 66.79 & 27.36 & 47.08 & 64.05 & 34.56 & 49.31\\


% \textbf{Ours (w/o trans.)} & Inductive & \textbf{74.58} & \textbf{34.99} & \textbf{54.79} &  \textbf{74.86} & \textbf{50.34} & \textbf{62.60}\\

% \hline
% RePRI~\cite{boudiaf2021few} \ \tt{(CVPR21)}  & Transductive & 20.76 & 10.50 & 15.63 &  34.06 & 20.98 & 27.52\\

% DIaM~\cite{hajimiri2023strong} \tt{(CVPR23)} & Transductive & 70.89 & 35.11 & 53.00 &  70.85  & 55.31 & 63.08\\

% \textbf{Ours (w trans.) }& Transductive & \textbf{76.39} & \textbf{39.83} & \textbf{58.11} &  \textbf{76.42} & \textbf{56.12} & \textbf{66.27}\\

% \tabucline[1pt]{-}
% \end{tabu}
% \end{adjustbox}
% \captionsetup{labelfont=bf}
% \captionof{table}{{\bf Comparison to state-of-the-art methods on PASCAL-$5^i$.} w/o trans., w trans.: without transduction and with transduction resp.}
% \label{tab:pascal}
% \end{table*}



\begin{table}[t]
     \centering
     \aboverulesep=0ex
     \belowrulesep=0ex
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{lc|c|c|c|c|c}
        \toprule
        
           &  \multirow{2}{*}{Causal Attention} & \multirow{2}{*}{Prompt Initialization} & \multirow{2}{*}{Transduction} & \multicolumn{3}{c}{mIoU}\\\cmidrule(r{2pt}){5-7}
          &  & & &  Base & Novel & Mean \\
        \midrule
      \textbf{(1)} & None & Random & No & 50.18 & 11.22 & 30.70\\ 
        % Random  &\scriptsize{None}  &   \scriptsize{-}  & 50.18 & 11.22 &  30.70   \\

    \textbf{(2)} & None  &   Masked Pooling    &   No  & 50.43 & 11.31 &  30.87  \\

   \textbf{(3)}  &  First Layer Only  &   Masked Pooling    &  No  & 51.53 & 12.26 &  31.90  \\
   \textbf{(4)} &   Separate Weights  &  Masked Pooling   &    No  & 51.06 & \underline{18.05} & 34.56   \\ 

    \textbf{(5)} & Shared Weights  &  Random   &  No  & 50.75 & 17.41 &  34.08   \\
    \textbf{(6)} & Shared Weights  &  Masked Pooling   &    No  & \underline{51.55} & 18.00 &  \underline{34.78}   \\ 
      
   \textbf{(7)} &  Shared Weights  &  Masked Pooling  &  Yes & \textbf{53.80} & \textbf{18.30} &  \textbf{36.05}   \\  
        \bottomrule
      \end{tabular}
  \end{adjustbox}
  \vspace{-4pt}
     \caption{{\bf Ablation Study on COCO-$20^i$.} The 1-shot performane, averaged over all folds.}
     \label{tab:ablation}
\vspace{-1.5em}
\end{table}




\subsection{Dataset and Implementation Details}
\label{sec:implementation_details}
\noindent
{\bf Datasets.} We evaluate our method on two few-shot segmentation benchmarks~\cite{tian2022generalized}: COCO-$20^i$ and PASCAL-$5^i$. Following~\cite{hajimiri2023strong} we report average performance of our model on 10K test images for COCO-$20^i$ and on all available test images on PASCAL-$5^i$. The results are reported as an average across five different runs on four different splits. 

\vspace{0.03in}
\noindent
{\bf Data Pre-processing.} We adopt the same setup as DIAM~\cite{hajimiri2023strong} for training the base model and fine-tuning on novel categories. During base training, images containing both base and novel categories are not removed from the training set; instead, the pixels corresponding to novel classes are relabelled as background. This approach, as highlighted by~\cite{hajimiri2023strong}, introduces challenges due to the potential ambiguity when the base model predicts novel categories as background. In fine-tuning, only novel classes are labeled in the support set, with base classes marked as background. Images with multiple novel categories are excluded from the support set to prevent unfair shot increases.

% We follow the same setup as DIAM~\cite{hajimiri2023strong} for both training the base model and fine-tuning on novel categories. In this setup, during base training, if an image containing base categories also contain a novel category, it is not removed but rather the pixels of novel classes are relabelled to background.  As argued by~\cite{hajimiri2023strong}, this presents a challenging setting because of the ambiguity that may arise in forcing the base model to predict potential novel categories as background. During fine-tuning, only novel classes are labeled in the support set while the base classes are labelled as background. Images with more than one novel category are not used as support images to prevent unfair shot increases.

% Following DiAM~\cite{hajimiri2023strong}, during training of the base model, we do not remove images that contain novel classes and any pixels belonging to novel classes are labelled as background. As noted in ~\cite{hajimiri2023strong}, this setting poses greater challenge because of the ambiguity that arises in forcing the network to predict potential novel categories as background. Similarly, following ~\cite{hajimiri2023strong}, during fine-tuning on novel classes, we label any pixel belonging to base classes as belonging to the background. Therefore in the support set, only the novel classes are labelled and the rest are treated as background. Care must also be taken to ensure that a support image does not contain more than one novel category, because it would unfairly increase the number of shots for that particular novel category. 
\vspace{0.03in}
\noindent
{\bf Evaluation Protocol.} We evaluate performance using the standard mean intersection-over-union (mIoU) metric. Following~\cite{hajimiri2023strong}, the mean score for generalized few-shot segmentation is computed as the average between \emph{base} and \emph{novel} mIoUs. This approach addresses bias in datasets like PASCAL-$5^i$ and COCO-$20^i$, where base classes outnumber novel classes threefold.

\vspace{0.03in}
\noindent
{\bf Implementation Details.} Our feature extractor is based on PSPNet~\cite{zhao2017pyramid} with Resnet-50~\cite{he2016deep}. We utilize the pixel decoder from Mask2Former~\cite{cheng2022masked}, based on MSDeformAttn~\cite{zhu2020deformable}. The dimension $C$ for visual prompts is chosen to be $256$. Contrary to \cite{cheng2022masked}, the base model is trained with 
per-pixel cross-entropy loss. We use AdamW optimizer~\cite{loshchilov2018decoupled} with base learning rate of $1 \times 10^{-4}$, a weight decay of $0.05$ and a batch size of $16$. 
%Following~\cite{lang2022learning, hajimiri2023strong}. 
Following~\cite{lang2022learning, hajimiri2023strong}, we train base model for 20 epochs for COCO-$20^i$ and 100 epochs for PASCAL-$5^i$. 

During novel fine-tuning, the parameters of the feature extractor, pixel decoder, and base segmentation head are frozen, while only the parameters of the visual prompts, novel segmentation head, and novel-to-base causal attention module are optimized. For inductive case, the model is fine-tuned with per-pixel cross-entropy loss for 100 iterations using AdamW optimizer with a learning rate of $5 \times 10^{-3}$ and a weight decay of 0.05. For transductive prompt-tuning, the model is first fine-tuned for 40 iterations with only cross-entropy loss to get a better marginal distribution and then fine-tuned for 60 more iterations with  full transductive losses mentioned in Eq.~\ref{eq:transduction}. The hyper-parameters  $\alpha$ and $\gamma$ are set to be 
100 and 25 respectively.

% % we apply per-pixel cross-entropy loss for the images in the support set. 

% We use AdamW optimizer with a learning rate of $5 \times 10^{-3}$ and a weight decay of 0.05.  We fine-tune the model for 100 iterations.

% For transductive prompt-tuning, we apply only cross-entropy loss for the first 40 iterations. We then update the marginal distribution estimate and train the model for 60 more epochs using the full transductive losses in Eq.~\ref{eq:transduction}. We set the values of hyper-parameters $\alpha$ and $\gamma$ in Eq.~\ref{eq:transduction} to be 100 and 25 respectively.


% \vspace{-7pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Previous Loc. Fig.3,4

\subsection{Results}
\vspace{-4pt}
\noindent
{\bf Comparison with the State-of-The-Art.} Table~\ref{tab:coco} compares the performance of our approach in both {\em inductive} and {\em transductive} setting against the state-of-the-art generalized few-shot segmentation (GFSS) approaches. As can be seen, our model outperforms existing approaches on both datasets. Interestingly, our approach, in an inductive setting (where optimization is performed only using a supervised few-shot support set, and evaluation is conducted on all test images), outperforms transductive GFSS approaches like DIaM~\cite{hajimiri2023strong} for both 1-shot and 5-shot cases on the COCO-$20^i$ dataset, which consists of 80 classes (60 base, 20 novel) and for the 1-shot case on Pascal-$5^i$, which has 20 classes (15 base, 5 novel). This is notable despite transductive approaches requiring test-time optimization for each unlabeled test image separately, leading to significantly longer inference times.


For a fair comparison in the {\em inductive} setting, we fine-tuned DIaM without the transduction losses and observe that % compared to the inductive setting for DIaM, 
our inductive approach has 5.78\% higher mIoU for 1-shot and 11.16\% higher mIoU for 5-shot on COCO-$20^i$. For PASCAL-$5^i$, the improvement from inductive DIaM is 7.71\% for 1-shot and 13.29\% for 5-shot. In fact, compared to the best inductive GFSS approach BAM~\cite{lang2022learning}, our inductive setting achieves an improvement of approximately 2.78\% and 7.59\% for 1-shot and 5-shot respectively on COCO-$20^i$ and 5.24\% and 12.32\% for 1-shot and 5-shot respectively on PASCAL-$5^i$. In comparison to the transductive DIaM~\cite{hajimiri2023strong} our inductive setting improves the mIoU by 2.03\% and 2.28\% for 1-shot and 5-shot respectively on COCO-$20^i$; for PASCAL-$5^i$ it is 
% sees an improvement of 
1.79\% higher, in 1-shot, than transductive DIaM~\cite{hajimiri2023strong}.
% while being only marginally lower (0.48\%) for 5-shot. 

We can further observe that when we perform {\em transductive} fine-tuning, the overall mIoU shows considerable gain outperforming transductive DIaM~\cite{hajimiri2023strong} in both 1-shot and 5-shot inference for both datasets. The improvement over DIaM for COCO-$20^i$ is 3.3\% for 1-shot and 3.93\% for 5-shot. For PASCAL-$5^i$, our transductive setting outperforms DIaM by 5.11\% and 3.15\% for 1 and 5-shots. % evaluation.
%\vspace{-2pt}

\begin{figure}[t]
    \centering
    %\vspace{-0.2in}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=0.5\textwidth]{sec/images/confusion_matrix.pdf}
    % \vspace*{5mm}
    \vspace{-0.1in}
    \captionof{figure}{{\bf Confusion Matrix for:} (left) model with Novel-to-Base Causal Attention; (right) model without Novel-to-Base Causal Attention. \leon{Note that Novel-to-Base Causal Attention reduces confusion between novel and base categories (bottom-left block).}}
    \label{fig:confusion_matrix}
    \vspace{-0.25in}
\end{figure}

\begin{figure}[t]
    \centering
    %\vspace{-0.2in}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=0.5\textwidth]{sec/images/TSNE.pdf}
    % \vspace*{5mm}
    \vspace{-0.2in}
    \captionof{figure}{{\bf TSNE visualization of the learned base and novel prompt features:} (left) with Novel-to-Base Causal Attention; (right) without Novel-to-Base Casual Attention. }
    \label{fig:tsne}
    \vspace{-0.10in}
\end{figure}


\subsection{Ablation} We performed a series of ablations, as shown in Table~\ref{tab:ablation}, to explain our design choices and the contributions of different components. 

\vspace{0.03in}
\noindent \textbf{Visual Prompts Initialization.} As seen in \textbf{(1)} and \textbf{(2)} of the Table~\ref{tab:ablation},  initializing novel prompts with masked mean pooling from the support set images improves both base and novel class accuracy compared to random initialization. This is more pronounced with novel-to-base causal attention~\textbf{(5)}--\textbf{(6)}, amplifying the performance gain from masked pooling initialization. 

% \textbf{Visual prompts initialization.} As can be seen from \circled{1} and \circled{2} of the table, initializing the novel prompt with masked mean pooling from the images of support set leads to better base and novel class accuracy than initializing the novel queries randomly. It is more apparent when there is novel-to-base causal attention \circled{5} as the gap in performance gain from masked pooling initialization increases.

\vspace{0.03in}
\noindent \textbf{Novel-to-base Causal Attention.} 
As seen in \textbf{(4)}--\textbf{(7)} of Table~\ref{tab:ablation}, novel-to-base causal attention yields the most significant improvement in novel class accuracy compared to \textbf{(1)}--\textbf{(2)}. This aligns with our hypothesis that uni-directional causal attention between rich base prompts (learned with many examples) and novel prompts (learned with few examples) increases separation among novel classes and pushes the feature space of base prompts away from the novel prompts. It is further confirmed by Figure~\ref{fig:confusion_matrix} and Figure~\ref{fig:tsne}. As observed in Figure~\ref{fig:confusion_matrix}, the novel-to-base causal attention leads to lower confusion between base and novel classes. Figure~\ref{fig:tsne} shows a t-SNE~\cite{van2008visualizing} visualization of the features of base and novel visual prompts for $10$ different test images. As observed, the incorporation of novel-to-base causal attention leads to much clearer separation of visual prompt features, particularly for novel prompts.

% As seen in \circled{4}-- \circled{7} of Table~\ref{tab:ablation}, it is the novel-to-base causal attention that leads to the biggest improvement in the novel class accuracy (compared to \circled{1}-- \circled{2}) . This matches our hypothesis that a uni-direction causal attention between the rich base prompt, learned with lots of examples, and novel prompt, which are learned with few examples, leads to a better separation between the novel classes. Moreover, it pushes the feature space of the base prompts away from novel prompts. We can observe similar pattern Figure~\ref{fig:confusion_matrix}. The model without the unidirectional novel-to-base causal attention tends to confuse the novel classes with base classes more often compared to the model with the causal attention. We also visualize the base and novel visual query features of the final layer for ten different test examples with and without causal attention as shown in Figure~\ref{fig:tsne}. As observed, the visual prompts representing individual classes are clearly separated from one another in the model with novel-to-base causal attention. For the model without the causal attention, we particularly observe that the novel query embeddings are cluttered and poorly separated from one another leading to poor novel class accuracy. 
\vspace{0.03in}
\noindent \textbf{Multiscale Causal Attention.} We also ablated the placement of the causal attention module. We observe that applying it only at the first layer \textbf{(3)}, slightly improves novel mIoU compared to the model without causal attention. Yet, it is notably inferior to applying at every decoder layer \textbf{(4)}-- \textbf{(7)}. We could have opted for separate parameters for the causal attention module at each layer. However, as seen in \textbf{(4)}, having separate weights offers little improvement to novel mIoU despite significant increase in total number of parameters to optimize. In fact, it decreases the base accuracy, leading to overall worse performance. 

%\vspace{0.03in}
\begin{figure}[t]
    \centering
    %\vspace{-0.2in}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=0.5\textwidth]{sec/images/qual_fig.pdf}
    %\vspace{-2em}
    \captionof{figure}{{\bf Qualitative Results} The leftomost two columns show image and ground truth mask; (Third) Baseline without causal attention; (Fourth); Ours in inductive setting; (Fifth) Ours in transductive setting; (Last) DIaM~\cite{hajimiri2023strong}. \leon{Last row illustrates a {\em failure}.} }
    \label{fig:qual}
\vspace{-8pt}
\end{figure}
\noindent \textbf{Qualitative Results.} Figure~\ref{fig:qual} compares the qualitative results of our proposed model in both inductive and transductive settings with the baseline lacking causal attention and the transductive DIaM~\cite{hajimiri2023strong}. Notably, for first row, both our inductive and transductive approaches predict more accurate segmentation of the \emph{cow} compared to DIaM. In second row, the causal attention improves \emph{person} segmentation followed by transduction. In the third row, DIaM completely misses the novel category \emph{chair}. The causal attention allows our model to better differentiate the base class \emph{dining table} from the novel class \emph{chairs}. Transduction improves accuracy of the segmentation of \emph{dining table}. In fourth row, we can observe that both DIaM and our model without causal attention misdetects novel class \emph{cat} for \emph{cow} at multiple locations. Causal attention allows our model to make a uniform and more accurate prediction of \emph{cat}. In the fifth row, we observe that DIaM~\cite{hajimiri2023strong} completely misses detecting the base category \emph{potted plant} and poorly segments \emph{person}. The baseline without causal attention misdetects the \emph{potted plant} with novel class \emph{bus} and misdetects \emph{dining table} with \emph{chair}. Causal attention improves the accuracy which is further improved by transduction. Last row demonstrates a case where our model performs worse than DIaM~\cite{hajimiri2023strong}. Here, again, we observe that adding causal attention reduces misclassification of \emph{person} with \emph{car}, although overall the segmentation of \emph{car} is less accurate than DIaM~\cite{hajimiri2023strong}.

% It has poor segmentation results and misdetections for class person, while our model without causal attention misdetects the potted plant with novel class bus and misdetects dining table with chair. Adding causal attention improves accuracy which is further improved in the transductive setting. We also show a failure case of our model (last image) and a case where DIaM performs better than ours. Again we can see adding novel-to-base causal attention reduces misclassification of person with car. However, the overall segmentation of the car is poor compared to DIaM. 

From the qualitative results, the effectiveness of novel-to-base causal attention at distinguishing base from novel classes becomes apparent. Our model in inductive setting outperforms transductive DIaM in most cases, despite the inference time being faster.

\vspace{-6pt}


% \textcolor{red}{We need specific commentary on the qual  examples.} 


==> sec/method_original.tex <==

As mentioned, we perform prompting using a set of learnable visual prompts, where, intuitively\footnote{This may not be precisely true in practice, but is a reasonable abstraction for intuitive understanding.}, each prompt corresponds to a class \leon{embedding}. These learned visual prompts cross-attend with image features at multiple scales. Initially, we pre-train a base model with abundant examples of base classes, learning visual prompts for them. We then fix these base prompts and fine-tune visual prompts for novel classes with a few examples. However, learning visual prompts with few examples is difficult since it often leads to confusion between base and novel categories. To allow more robust learning and improve novel class generalization, we introduce a uni-directional causal attention mechanism between novel and base prompts. Intuitively this allows better contextualization and repulsion / attraction  
between base and novel prompts. As we show in Section~\ref{sec:exps} this mechanism proves highly effective empirically. 



% As mentioned, 
% % we aim to design a non-meta learning approach to training visual prompts with few-shot examples. 
% % \leon{[Why aim for non-meta learning? We either need to motivate this or not state this as explicit aim.]}
% we perform visual prompting through a set of learnable visual queries (or embeddings) 
% where, intuitively\footnote{This may not be precisely true in practice, but is a reasonable abstraction for intuitive understanding.}, each visual query 
% corresponds to a particular class \textcolor{red}{or attribute}. These learned visual prompts queries \jim{do you want both prompts and queries?}
% are used to cross-attend with image features at multiple scales.
% % prompt the image features at multiple scales.
% To that end, we first pre-train a base model with abundant examples of base classes and learn a set of visual queries for the base classes. 
% We then fix these base prompts and learn visual prompts for the novel classes by 
% % adding new visual queries for the novel classes and 
% fine-tuning them with few examples. 
% However, learning visual prompts using few-examples tends to be difficult, and often results in confusion between base and novel classes. 
% To facilitate more robust learning that improves novel class generalization, we introduce uni-directional causal attention mechanism between the novel and the base prompts. Intuitively this allows better contextualization and repulsion / attraction  
% between (fixed) base and fine-tuned novel queries (or embeddings).
% As we show in Sec.~\ref{sec:exps} this proves very effective in practice. 

% Fig~\ref{fig:model} illustrates the overview of proposed approach. 

% To facilitate the rich features learned by the base visual queries, we apply a uni-direction causal attention mechanism between the newly added novel queries and the abundantly learned base queries. This directional causal attention allows the base queries to enhance the features of novel query features enabling capturing semantic relationship between the classes. Fig~\ref{fig:model} shows the overview of our proposed approach. 

% In what follows, we will first describe the learned visual queries and how they used to prompts image features at different scale in the proposed architecture. Then we will describe the proposed unidirectional causal attention between learned base and novel queries followed by the base training and novel fine-tuning steps. At the end we will discuss how we can adopt our proposed method to allow transductive prompt tuning for novel queries by utilizing the unlabelled test images. 

% \subsection{Learnable Multi-scale prompts}
% Figure~\ref{fig:model} shows our proposed architecture in details. At the core of our approach are the learnable embeddings, which we term {\em visual prompts}, that are used to prompt the image features at multiple scales. The design of our segmentation architecture is inspired by Mask2former~\cite{cheng2022masked} with couple of key differences: (i) the number of learned visual queries is tightly coupled with the number of classes, where each visual query is representative of a class and can be thought of as a learned embedding for that class; (ii) we perform per-pixel classification, instead of mask-classification, thereby getting rid of the query classification component of \cite{cheng2022masked} and instead defining custom segmentation heads.  

Figure~\ref{fig:model} shows our proposed architecture. It centers around learnable embeddings called \emph{visual prompts}, which \leon{interact with} image features at multiple scales. Our design is inspired by Mask2former~\cite{cheng2022masked} with a couple of key differences: (i) the number of visual prompts aligns with the number of classes, each representing a class as a learned embedding; (ii) we adopt per-pixel classification, instead of mask classification, thereby eliminating the query classification component of \cite{cheng2022masked} and defining custom segmentation heads \leon{capable of making per-pixel predictions}.

\subsection{Visual Prompting Multiscale Transformers} ~\label{subsec:base}
\hspace{-4pt}\noindent {\bf Base Visual Prompts.} Given $B$ base classes, we define $B$ visual prompts each representing a class and initialize them randomly. These visual prompts, first self-attend to learn the relationship between themselves and then are used to prompt the image features at multiple scales. The refinement of base prompts at each decoder layer is given by: 
%
\begin{equation}
    V_B^{(l)} = \mathcal{A}(V_B^{(l-1)}) + \mathcal{C}(V_B^{(l-1)}, F^{(l-1)}),
\end{equation}
%
\noindent
where $\mathcal{A}$ and $\mathcal{C}$ refer to multi-headed self and cross attention respectively; $V_B^{(l)} \in \mathbb{R} ^{B \times C} $ are the base visual prompts at layer $l$; $ F^{(l)} \in \mathbb{R}^{H_l W_l \times C_l}$ is the flattened image feature at layer $l$; $H_l$ and $W_l$ denote image dimensions at that layer; $C_l$ denotes the embedding dimension. 

Once the prompts are refined, through multiple levels of transformer attention, a segmentation head is defined that makes per-pixel predictions. This segmentation head, $\mathcal{H}(\cdot)$, takes as input the final refined prompts, $V_{B}^{(L)}$ and the highest resolution image features, $F^{(L)}$, and outputs per-pixel per-class predictions $O_{base} \in \mathbb{R}^{B\times H\times W}$ \leon{(see Section~\ref{sec:seghead})}.

\vspace{0.1in}
\noindent
{\bf Novel Visual Prompts.} 
Once the model is trained on the base classes, we freeze all the layers of the model except the visual prompts representing the base-classes. Given there are $N$ novel classes, we add $N$ new visual prompts. We further add a causal unidirectional attention module that allows the the novel prompts to be enhanced by the base prompts.  The details of this module are provided in Section~\ref{subsec:base_to_novel}. 
The output is similarly passed to a segmentation head to then make predictions for the novel classes.

The novel visual prompts are first refined by unidirectional novel-to-base causal attention module. These enhanced novel prompts are then concatenated with the base prompts and enhanced in the manner similar to base prompts. This is given by:
%
\begin{eqnarray} 
    V_N^{(l)} & = & \mathcal{CA}(V_B^{(l)}, V_N^{(l)}) \nonumber \\
    V_A^{(l)} & = & \left[ V_B^{(l)},  V_N^{(l)} \right] \nonumber \\
    V_A^{(l)}  & = & \mathcal{A}(V_A^{(l-1)} ) + \mathcal{C}(V_A^{(l-1)}, F^{(l-1)}), \nonumber
\end{eqnarray}
%
where $V_N^{(l)} \in \mathbb{R}^{N \times C} $ are novel prompts at layer $l$; $N$ is the total number of novel class and $C$ is the embedding size; $V_A^{(l)} \in \mathbb{R}^{(B+N)\times C} $ are all visual prompts including base and novel; $\left[.,.\right]$ is the concatenation operator. The operation $\mathcal{CA}$ denotes the causal novel-to-base attention and is explained in Section~\ref{subsec:base_to_novel}. 

Each of the $N$ novel visual prompts (representing a novel class) is initialized using masked average global pooling of the k-shot support images corresponding to the class masked by the ground truth binary masks. %For k-shot case, we simply take the mean of the masked average features across the k-examples: 
%
\begin{equation} \label{eq:init}
    V_n^{(0)} = \frac{1}{K}\sum\limits_{k=1}^K \frac{\sum\limits_{x, y} {M^k_n}(x, y) F^k_n(x, y)}{\sum\limits_{x, y} M^k_n(x, y)}, \forall n \in N
\end{equation}
%
where $V_n^{(0)} \in \mathbb{R}^{1 \times C}$ is the initial novel visual prompt for novel class $n$; $F^k_n$ denotes the image features of $k$-th shot for novel class;  $M_n^k$ denotes the corresponding ground-truth binary mask; $x, y$ are the spatial locations; $N$ is the total number of novel classes and $K$ is the total number of shots. %The operator $\circ$ denotes element-wise multiplication. 

\subsection{Novel-to-base Causal Attention}\label{subsec:base_to_novel}
% \rayat{Although the base and novel categories by themselves are independent, the latent visual prompt representing the base and novel categories can confound one another.}
A key component of our proposed approach is the uni-directional novel-to-base prompt causal\footnote{We use the term {\em causal} borrowing from its use in the look-ahead-attention-masking for decoder Transformers~\cite{vaswani2017attention} ({\em e.g.}, in language)} attention. The base visual prompts are learned with abundant examples; this is not the case for novel prompts. Learning novel prompts directly or having novel prompts impact the base ones could therefore lead to degradation of performance. However, having novel prompts aware of their base counterparts could be quite helpful. We hypothesize that causal attention between the novel visual prompts and base prompts could help contextualize novel class embeddings, reducing confusion with the base counterparts.  Motivated by this intuition, we propose a novel-to-base causal attention layer that is repeated at each scale (or layer of the transformer decoder); see Fig.~\ref{fig:model}.    
% \rayat{Due to this disparity between the amount of data used to learn the query representations, the confounding effect of base queries on the novel queries are more significant especially if the novel queries are to be learned on its own. We hypothesize that an unidirectional causal attention between the base and novel visual queries, where the base queries are treated as confounding variables to better contextualize novel class embeddings, would reduce confusion with the base counterparts, which in-effect would improve both novel and base class prediction. Motivated by this intuition, we propose a unidirectional novel-to-base causal attention layer, where base queries are considered as confounding variable to enhance the novel queries. This module is repeated at each scale (or layer of the transformer decoder); see Fig.~\ref{fig:model}. } 
% Learning novel queries directly or having novel queries impact the base ones could therefore lead to degradation of performance.  However, having novel queries aware of their base counterparts could be quite helpful.
% We hypothesize that causal attention between the novel visual queries and base queries could help contextualize novel class embeddings, reducing confusion with the base counterparts.  

% Motivated by this intuition, we propose a novel-to-base causal attention layer that is repeated at each scale (or layer of the transformer decoder); see Fig.~\ref{fig:model}. 
% As seen in Fig~\ref{fig:model}, this Novel-to-base causal attention layer is repeated to refine the novel queries at every layer of the decoder.

The proposed causal attention module is a single layer cross-attention where the Key $K^{(l)}$, Value $V^{(l)}$ and $Q^{(l)}$ for layer $l$ of the decoder are given by: 
\begin{equation}
    Q^{(l)} = V_N^{(l)}  W^Q; ~~~~K^{(l)} = V_B^{(l)}  W^K; ~~~~V^{(l)} = V_B^{(l)} W^V \nonumber
\end{equation}
%
where $W^Q, W^K , W^V$ are weight matrices for $Q$, $K$ and $V$ respectively. The parameters $W^Q $, $W^K $, $W^V $ are shared at all the layers of this cross-attention module to reduce the number of trainable parameters during fine-tuning on novel classes to prevent overfitting and poor generalization. 

This uni-directional novel-to-base causal attention refines the novel visual prompts $V_N^{(l)}$ at each decoder layer $l$ by:
%
\begin{equation}
    V_N^{(l)} = \mathrm{softmax} (Q^{(l)} (K^{(l)})^\mathrm{T} ) V^{(l)} \nonumber
    \end{equation}
%
The resulting product of this module are a set of refined and contextualized novel visual prompts. % capturing the semantic similarities and relationships.

\subsection{Segmentation Head}
\label{sec:seghead}
\noindent
{\bf Base Segmentation Head.} 
The base segmentation head, $\mathcal{H}_B$, during the base training in the proposed model is relatively simple and takes the form of a three layer MLP that projects a refined prompt into, effectively, class prototype; computes the (dot product) similarity of each pixel feature with that prototype, and then applies softmax along the channel / class dimension to obtain per-pixel and per-class probability: 
%\mathrm{softmax}\left( \right)
\begin{eqnarray} \label{eq:base_output}
    O_{base} & = & \mathcal{H}_B(V_{B}^{(L)}, F^{(L)}) \nonumber \\ 
             & = &  \mathrm{MLP}\left(V_{B}^{(L)}\right) \cdot \left[F^{(L)}\right]^\mathrm{T},
\label{eq:baseseghead}
\end{eqnarray}
%
where $O_{base} \in \mathbb{R}^{B\times H\times W}$ and the class assignment can then be made by an $\mathrm{argmax}$ along the channel dimension. 

% \leon{[There is no softmax or anything on top of $O_{base}$?]}

%\vspace{0.1in}
%\noindent
%{\bf Base Learning Objective.} The model is trained using a simple per-pixel cross-entropy loss on abundant base data.

\vspace{0.1in}
\noindent
{\bf Novel Segmentation Head.}
While we could, in principle, use the same form of segmentation head during few-shot inference as that defined for the base classes (see Eq. \ref{eq:baseseghead}), simply fine-tuning it for novel classes, this proves ineffective in practice. 
Specifically, fine-tuning the MLP leads to significant overfitting given the few examples and lack of base class data during this step. 
% this proves to not be effective as number of parameters in MLP is too large resulting in over-fitting and poor performance in practice when optimized with few examples. 
So, instead, we resort to a simpler form of the novel segmentation head, $\mathcal{H}_N$, where we only learn a residual to the MLP learned during base training (which we keep fixed), mainly:
%
% Additionally, in order to appropriately segment the novel classes, we add a separate segmentation head which we call {\em novel} segmentation head. It is necessary because the parameters of the base segmentation head has been trained with lots of data and it is difficult to achieve a good generalization on novel classes from few examples.
%
% Overall the output for the novel classes is obtained by passing the novel visual queries and the final layer image features to the novel segmentation head. This is given by: 
%
\begin{eqnarray}
    O_{novel} & = & \mathcal{H}_N(V_{N}^{(L)},  F^{(L)}) \nonumber \\
    & = & \left[ \mathrm{MLP}_{\bullet} (V_N^{(L)}) + W_N \right] \cdot \left[F^{(L)}\right]^\mathrm{T} , \nonumber
\end{eqnarray}
%
where $O_{novel}$ is output for novel classes and $\bullet$ designates that parameters of MLP are frozen and only $W_N \in \mathbb{R}^{N \times C}$ weight matrix is learned.
% ; $I$ is the query image; $V_N^{(L)}$ are novel visual queries of the last layer decoder layer $L$; and and $W_N$ is the weight vector for the novel segmentation head. 
This weight matrix is initialized in the same manner as novel prompts, in Eq.~\ref{eq:init}. 
% The function $\sigma_{mlp}(.)$ is the same MLP function defined in equation~\ref{eq:base_output} and its parameters remain frozen during novel fine-tuning. \leon{I am confused, I thought we were not doing MLP for novel classes :/}

%\vspace{0.1in}
%\noindent
%{\bf Novel Learning Objective.} The parameters of visual query embeddings, novel-to-base causal attention module and the novel classification head are learned using the few-shot examples in the support set using per-pixel cross entropy. All other parameters are frozen at base training values. 

\subsection{Transductive Prompt Tuning} \label{subsec:transduction}


Recent approaches like DIaM~\cite{hajimiri2023strong} and RePRI~\cite{boudiaf2021few} highlight the effectiveness of a good transductive setting for few-shot dense prediction tasks. Transductive approaches perform test-time optimization for each unlabeled test image and utilize specific characteristics and information of the test instances to improve prediction.

 % In transductive learning, the model takes into account the specific characteristics of the test instances during the prediction phase, leveraging information from both labeled and unlabeled data at test time. 

% However, this approach, involving test-time optimization for each unlabelled test image which leads to slower inference despite performance gains (since inference is no longer feedforward). \leon{[Why talking about inference speed here is important? It would be slow for any transductive method and is completely orthogonal to our approach or contributions. I would simply remove the last sentence. If we want to discuss inference speed between inductive and transductive settings, we should do that in the result section.]}

% Recent approaches like DIaM~\cite{hajimiri2023strong} and RePRI~\cite{boudiaf2021few} have shown that a transductive setting could be very effective for few-shot dense prediction tasks. Transductive inference involves test-time optimizing of the model for each unlabelled test image. Despite improved performance, one downside of transductive inference is slower runtime (since inference is no longer feedforward). 
%

To demonstrate the flexibility of the proposed approach, we describe, in this section, how our model can be adapted for transductive inference to achieve even stronger GFSS performance through transductive fine-tuning of the visual prompts. We build on the transductive losses proposed in DIaM~\cite{hajimiri2023strong}  and we describe them here for completeness. 

The losses are designed to maximize the mutual information between the learned features and the corresponding predictions on the test image, which is achieved through maximizing: 
$\mathrm{H}(O) - \mathrm{H}(O | I)$, where $I, O$ are random variables associated with the pixels and predictions distributions respectively; $\mathrm{H}(O)$ is the marginal  and $\mathrm{H}(O | I)$ is the conditional entropy.
%
The conditional entropy $\mathrm{H}(O|I)$ involved is given by sum of cross-entropy loss over the supervised support set and entropy of the predicted probability given the test image $I$. The marginal entropy is given by KL divergence loss relying on an estimated region proportion prior following~\cite{boudiaf2021few}. Additional details are in \cite{hajimiri2023strong}.

% and support set images $|S|$ : 
% 
% \begin{equation} \label{eq:entropy}
%     \mathrm{H}(Y|X) = \mathrm{H}(P(X)) +\alpha \sum_{i \in |S|} L_{\mathrm{CE}}(P(i), T_i)  
% \end{equation}
% 
% Where $T_i$ is the ground truth labels for image $i$ in the support set $|S|$ and $P(X)$ is the prediction for the query image;  $L_{\mathrm{CE}}(P(i), T_i)$ is per-pixel cross-entropy loss and $\alpha$ is a controlling hyper-parameter.
% 
% 
% The marginal entropy $\mathrm{H}(Y)$ is given by: 
% 
% \begin{equation}
%     \mathrm{H}(Y) = \mathrm{const.} - \mathrm{KL} ( \ Y || \ \mathbf{\Pi})
% \end{equation}
% 
% Where $ \ \mathbf{\Pi}$ is an estimate of the marginal distribution of the model and $\mathrm{KL}(.||.)$ indicates KL-divergence. 

In addition to the aforementioned losses, similar to~\cite{hajimiri2023strong}, we use knowledge-distillation loss to preserve base class performance. This loss is given by: 
%
\begin{equation}
    \mathcal{L}_{\mathrm{KD}} = \mathrm{KL} (O_{base}^{new} \ \ || \ \ O_{base}^{old}  ),
\end{equation}
%
where $O_{base}^{old}$ is the prediction probability of the base classes of the frozen model after base training; $O_{base}^{new}$  is the prediction probability of the base classes on the model with our additional components to handle novel categories that is being fine-tuned. These include the multiscale causal novel-to-base cross attention and the novel prompts.
%\leon{[check consistency of variables]}

The overall objective function to minimize during transduction is given by:
%
\begin{equation}  \label{eq:transduction}
    \mathcal{L}_{\mathrm{trans.}} = \alpha \mathrm{H}(O|I) - \mathrm{H}(O) + \gamma \mathcal{L}_{\mathrm{KD}},
\end{equation}
%
where $\alpha$ and $\gamma$ are balancing hyper-parameters.

In the transductive setting, we noticed that applying transduction from the first iteration underperforms, possibly due to an initially poor estimation of the marginal distribution. To address this, we only apply per-pixel cross-entropy loss for a set number of iterations. Once we achieve a more accurate estimate of the marginal distribution, we then incorporate the remaining transductive losses from Eq.~\ref{eq:transduction}.

% Due to the marginal entropy component $\mathrm{H}(Y)$, the performance over novel class is dependent on the initial marginal distribution $ \ \mathbf{\Pi}$ estimate. DIaM applies all three components from first iteration for a query image and update  $ \mathbf{\Pi}$ after a certain number of iterations and continue applying the losses. However, if the initial marginal distribution over the novel classes is poor, it leads to degenration of performance on novel classes.

% We observe that applying transduction from the first iteration leads to slightly worse performance on novel classes compared to simply applying cross-entropy loss over the support set. This is most likely due to poor estimation of the initial marginal distribution. Therefore, in a transductive setting we first finetune our novel prompts and corresponding parameters using per-pixel cross-entropy loss over the support set for a certain number of iterations. Once we have a better estimate of the marginal distribution over-classes, we start applying rest of transductive losses in Eq.~\ref{eq:transduction}.  

% We observed that applying transduction from the first iteration slightly underperforms compared to just using cross-entropy loss over the support set, likely due to poor inital estimation of the marginal distribution. Therefore, in the transductive setting, we first fine-tune novel prompts and parameters using per-pixel cross-entropy loss only for a certain number of iterations. After obtaining a more accurate estimate of the marginal distribution, we incorporate the remaining transductive losses from Eq.~\ref{eq:transduction}.


% we use cross-attention mechanism to interact with visual queries that represents the base classes, pre-trained with abundant examples, to enrich the novel visual queries

==> sec/related_slight_change.tex <==
\textbf{Few-shot Learning.} Few-shot learning has a long history in computer vision and has emerged as a paradigm to test data efficiency and adaptability of learning algorithms. It is formulated as aiming to make predictions on {\em novel} classes for which only few labeled examples are available, often by leveraging and transferring information from (disjoint) {\em base} classes for which abundant data exists.
Few-shot learning has been studied extensively in the context of image classification \cite{FinnICML2017,RaviICLR2017,RenICLR2018,snell2017prototypical,vinyals2016matching}. Most approaches can be categorized as either {\em transfer} or {\em meta}-learning-based. Transfer learning methods \cite{dhillon2019baseline} typically pre-train the model on base classes with abundant data and then fine-tune this model for novel classes with few samples. 
Meta-learning \cite{FinnICML2017,RaviICLR2017}, which has become the most dominant approach to few-shot learning to date, emulates the inference stage during training by sampling tasks of support and target sets. Meta-learning approaches can be sub-categorized into {\em gradient-based} and {\em metric-learning} based. Gradient-based approaches \cite{FinnICML2017,RaviICLR2017} learn the commonalities among different tasks. Metric-based (or prototype-based) ones \cite{snell2017prototypical,vinyals2016matching} learn image embeddings and compare the distances between them. Despite popularity and strong performance, issues with meta-learning in terms of sensitivity to the meta-training setup~\cite{cao2019theoretical} and worse performance with domain shift~\cite{chen2019closer} are observed.

Generalized few-shot learning, as a more realistic variant, was introduced in \cite{HariharanICCV2017} where the query images can be from either base or novel categories. Recently transductive setting has been proved to be effective for few-shot learning~\cite{boudiaf2020information, qi2021transductive, boudiaf2021few, hajimiri2023strong, zhu2023transductive}. 
%Unlike the inductive setting, discussed so far, in the inductive setting. 
There has been a rise in transductive inference mechanisms that allow for the use of the unlabelled target images to improve the classification~\cite{liu2018learning,nichol2018first,dhillon2019baseline,qiao2019transductive}. 
These approaches build on classic semi-supervised learning approaches, such as graph-based label propagation \cite{LiuICLR2019} or entropy minimization \cite{dhillon2019baseline}.
More recently variants of few-shot learning problems have also been established in other more granular domains, {\em e.g.}, detection \cite{Kang2019ICCV,WangICCV2019,YanICCV2019,WangICML2020} and segmentation.


% textcolor{red}{\textbf{Few-shot learning.} Few-shot learning is focused on improving the generalization ability of models to novel classes unseen during the initial training to classify the target images guided by few labelled examples, i.e., the support set. Most approaches emulate the inference stage during training by sampling tasks of support and target sets, referred to as meta-learning~\cite{snell2017prototypical,vinyals2016matching,Triantafillou2020Meta-Dataset}. However, multiple works discussed potential issues in terms of sensitivity to the meta-training setup~\cite{cao2019theoretical} and worse performance with domain shift~\cite{chen2019closer}. Recently, there has been a rise in transductive inference mechanisms that allow for the use of the unlabelled target images to improve the classification decision without meta-learning~\cite{liu2018learning,nichol2018first,dhillon2019baseline,qiao2019transductive}. Nonetheless, there exists less emphasis on few-shot learning in the context of semantic segmentation.}

\vspace{0.05in}
\noindent
{\bf Few-shot segmentation.}
While less prevalent, compared to classification, few-shot segmentation has been emerging as the new dense counterpart to approaches above. 
Few-shot segmentation approaches can be categorized to {\em prototype-based} and {\em dense comparison-based} methods. Prototype-based methods mostly relied on extracted prototypes from the support set to guide the segmentation of the target image, either as single prototype~\cite{zhang2019canet,wang2019panet}, part-aware~\cite{liu2020part} or a prototype mixture~\cite{yang2020prototype}. Dense comparison methods rely on dense comparisons between the few template images and the target image~\cite{yang2020brinet,zhang2019pyramid} with extension to multiscale~\cite{min2021hypercorrelation}. A recent approach was proposed for the generalized few-shot segmentation task where the unlabelled target images are used to improve the segmentation of novel classes while maintaining previous performance on base classes through knowledge distillation~\cite{hajimiri2023strong}. A concurrent work~\cite{liu2023learning} on generalized-few shot segementation learns a set of orthogonal proptotypes for base and novel categories, thereby aiming to reduce the influence of base-class prototypes to novel prototypes.~\cite{zhang2022feature} proposed a prompting strategy to segment foreground class from background from few-shot examples where a set of class-aware prompts are learned segment the foreground class. Crucially this approach is designed for 1-way segmentation only and performs prompting at a single scale unlike ours. 
% However, notably, none of the techniques so far have leveraged prompting. 
% However, previous methods in transductive inference did not reap the benefits of prompting. %Additionally, our method without transductive losses is still able to outperform that recent strong baseline on the generalized few-shot segmentation task.

% POP builds a set of orthogonal prototypes, each of
% which represents a semantic class, and makes the prediction
% for each class separately based on the features projected
% onto its prototype. Technically, POP first learns prototypes
% on base data, and then extends the prototype set to novel
% classes. The orthogonal constraint of POP encourages the
% orthogonality between the learnt prototypes and thus miti-
% gates the influence on base class features when generalizing
% to novel prototypes. 

%\vspace{0.05in}
\noindent
{\bf Prompting.} An emerging direction in learning with limited labelled data is to utilize foundation models that have strong generalization capabilities. Foundation models~\cite{bommasani2021opportunities} are pre-trained on large-scale data and adapted to downstream tasks showing generalization in few-shot settings~\cite{NEURIPS2022_960a172b}. Prompting is one promising direction to adapt these foundation models to few-shot tasks, where it formulates the inference problem similar to the training. One example~\cite{NEURIPS2022_960a172b} uses auto-regressive modelling ({\em i.e.}, predicting the next token given the previous ones). The inference in this case becomes a simple generation of the next tokens after receiving the correct prompt ({\em i.e.}, set of textual or visual tokens) the model is expecting. For few-shot learning, prompts include few-shot demonstrations followed by the query. In prompting we can either use discrete prompts~\cite{NEURIPS2022_960a172b} or learn continuous prompts~\cite{li2021prefix} through back-propagation. In computer vision, both vision-language prompting~\cite{NEURIPS2022_960a172b} and visual prompting~\cite{jia2022visual} of transformer-based models have shown promising success in various vision tasks, especially the few-shot ones. Yet, how to effectively prompt models that are designed for localization and segmentation is an open question. 

% Yet, it begs the question of how to prompt models that are designed for localization and segmentation tasks while relying on transformer decoders. 

%\textcolor{red}{We need to also add CORA (CVPR23) work as concurrent}
\vspace{0.05in}
\noindent
{\bf Concurrent Work.}
% Concurrent to our work, 
A recent method~\cite{bulat2023fs} proposed prompting of transformer decoders for few-shot object detection. While conceptually related, their approach is designed for a different task (detection) as compared to ours (semantic segmentation), trained within a meta-learning framework while ours does not require meta-learning.
Further, \cite{bulat2023fs} lacks novel-to-base attention which is at the core of our architectural design. 
% \textcolor{red}{More importantly, the aforementioned work is designed within a meta-learning scheme where prompts are conditioned on the image, thus might inherit drawbacks discussed earlier.}
A recent foundation model for semantic segmentation, SAM~\cite{kirillov2023segment}, has shown strong performance when prompted by point, bounding box or text. 
However, it is not specifically designed for few-shot inference, which may require fine-tuning with the support set and other non-trivial changes to~\cite{kirillov2023segment}.
More significantly, its utilization of extensive data, that encompasses a wide range of classes, makes it unsuitable for few-shot tasks, as it undobtedly seen many target classes in training. 
%
%
% textcolor{blue}{However, it is not specifically designed for few-shot inference with separate support set imagery. Moreover, its utilization of extensive data encompassing a wide range of classes makes it unsuitable for few-shot tasks, and its inability to allow prompt tuning renders it less adaptable.} 
%Notably, SAM~\cite{kirillov2023segment} . As discussed in MedSAM \cite{wu2023medical}, SAM~\cite{kirillov2023segment} performance on unseen categories or domain like medical images is worse compared to fine-tuning on the unseen images.}
% Dont refer to MedSAM better its too much because its not poorly it was still working but less than finetuning so avoid bring up MedSAM. 
%
% \textcolor{blue}{However, exploiting such models  might not be appropriate or relevant to few-shot segmentation because they are trained on huge amount of data and most likely may have seen and learned to segment any of the novel classes of interest. Moreover, SAM~\cite{kirillov2023segment} is not designed to handle few-shot inference. As shown by MedSAM~\cite{wu2023medical} SAM are not particular good at segmenting concepts or objects that it has not observed (like medical images) and thereby needs fine-tuning}  
% However, the setup and problem definition for Segment Anything \cite{kirillov2023segment} are quite different from the traditional few-shot scenarios we target. 
Beyond the differences mentioned above, which include multi-scale tranformer prompting and novel-to-base attention, our method is the first to explore transductive prompt-tuning where the visual prompts can be optimized further with the unlabelled target images.

% However, their scheme relied on meta-learning where they conditioned the visual prompts on features from the support set and pseudo-class embeddings. Yet, this may inherit some of the limitations of meta-learning as discussed earlier. A recent foundation model for semantic segmentation has shown superior performance prompted by point, bounding box or text~\cite{kirillov2023segment} from a human annotator. Nonetheless, it was designed to be prompted for the target image unlike the few-shot setup that allows to be guided by different imagery in the support set without a human annotator interference. Unlike previous methods, we propose to benefit from the heart of what prompting is (i.e., formulating the few-shot inference similar to what was occurring during training). We devise a novel prompting technique for transformer decoders without meta-learning, through looking upon the learnable queries as visual prompts that can similarly be constructed during few-shot inference. Novel visual prompts are constructed based on the few training examples during inference while learning cross attention to the previously trained visual prompts. The strength of our method is that it avoids the potential issues in meta-learning and allows for fine-tuning these novel continuous visual prompts. Additionally, our method is the first to explore transductive prompt-tuning where the novel visual prompts initialized from the support set can be leveraged further with the unlabelled target image itself. Finally, the flexibility of our method allows for its usage with multiscale transformer decoders benefiting from high resolution detailed features unlike previous work, through learning a hierarchical cross-attention between the novel and base prompts.

==> sec/supplementary_original.tex <==
\setcounter{section}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\thetable}{\Alph{table}} % Use letters for table numbering
\renewcommand{\thefigure}{\Alph{figure}} % Use letters for figure numbering

% \textcolor{red}{Please add another subsection for additional qualitative result if you can add from different splits as well.}

\begin{abstract}
This document provides additional material that is supplemental to our main submission. Section~\ref{sec:efficiency} describes the computational efficiency results. Section~\ref{sec:ablation} includes additional ablation studies. Section~\ref{sec:split_class_results} provides split and class-wise performance results, followed by Section~\ref{sec:multi-scale} that analyzes the performance on objects of varying size. Section~\ref{sec:add-qual} discusses additional qualitative results on COCO-20$^i$ dataset. Finally, Section~\ref{sec:societal} details the societal impact of our work as standard practice in computer vision research.
\end{abstract}

 \section{Computational efficiency comparison} 
 \label{sec:efficiency}
In Table 1 in the main submission, we demonstrated the superior performance of our approach, even in the inductive setting, outperforming transductive methods such as DIaM. Transductive approaches necessitate test-time optimization for each data example computing transductive losses, leading to higher inference times. As illustrated in Table~\ref{tab:params}, there exists approximately 20$\times$ increase in inference speed of our inductive approach compared to transductive methods like DIaM~\cite{hajimiri2023strong}. Another important observation is that while our model has a higher number of parameters overall, it is computationally efficient as the number of FLOPs is approximately 57\% lower. 

% While our method has greater number of model parameters than DIaM but with minimal increase with respect to gains in both speed and accuracy. 


 \section{Additional Ablation Studies}
 \label{sec:ablation}
 \subsection{Number of Training Iterations} In Figure~\ref{fig:iters}, we present a graph of how our performance varies in the inductive setting for  different number of training iterations. While the results reported in Table 1 of the main paper were evaluated after 100 training iterations, both inductive and transductive, the figure reveals that extending the optimization process to a higher number of iterations consistently enhances performance, peaking notably at 300 iterations, but at the expense of run-time.


\subsection{Transduction Ablation} As mentioned in Section 4.4 of the original paper, our observations indicate that incorporating transductive losses from the initial iteration results in sub-optimal mIoU on novel classes. This is attributed to inaccurate estimation of the label marginal distribution that is used in the transductive losses. To illustrate this, Figure~\ref{fig:start_trans} showcases the performance of our model in 1-shot inference within a transductive setting, varying the number of iterations at which transduction is applied. Notably, it demonstrates that applying transduction either early or late results in performance degradation.

\input{tables/runtime}
\input{graphs/iters}
\input{graphs/start_transduction}

\input{graphs/shots_base}
\input{graphs/shots_novel}

\subsection{Shots Analysis} We conducted an ablation to evaluate the performance of our model in an inductive setting, considering various shot configurations. We compared it with the baseline lacking novel-to-base causal attention and inductive DIaM (without transduction)~\cite{hajimiri2023strong}. 

In Figure~\ref{fig:shots_base}, we demonstrate the variation in base class performance across different shots. As observed, our method maintains a consistently high base class performance, peaking notably at 7-shot. In contrast, the model without causal attention exhibits a gradual decline in base class performance as the number of shots increases. Notably, inductive DIaM experiences a sharp decline in base performance with the growing number of shots. This observation underscores the robustness of our model in retaining base class performance as it encounters more examples of novel classes. 

Likewise, in Figure~\ref{fig:shots_novel}, we illustrate the change of novel class performance across a different number of shots. Notably, our model demonstrates a consistent improvement in novel class performance as the number of shots increases. In contrast, both the baseline without causal attention and inductive DIaM~\cite{hajimiri2023strong} exhibit a plateau in novel class performance around the 5-shot mark. In our model, the leap in performance between different shots is notably more pronounced, demonstrating its capacity for significant improvement with increasing number of examples of the novel class. 

\input{tables/splitwise}
\input{tables/classwise}
\input{tables/object_size}

\section{Split and Class-wise Results}
\label{sec:split_class_results}
\paragraph{Split-wise Results.} Adhering to the established few-shot segmentation protocol, our model undergoes evaluation across four distinct splits or folds for both the PASCAL-5$^i$ and COCO-20$^i$ datasets. Within each fold or split, a subset of the classes are reserved as novel, serving as the validation set. Results presented in the main manuscript represent an average across all four splits. For a detailed breakdown, Table~\ref{tab:splitwise} provides the performance of our model on each of the four splits individually for both datasets, in both inductive and transductive settings. As expected, the performance on novel classes improves substantially for 5-shot cases across all the splits. Additionally, transduction generally enhances both base and novel class accuracy, except for split-3 of COCO-20$^i$, where the novel class performance experiences a minor degradation, although the base class performance increases.

\begin{figure}[t]
    \centering
    %\vspace{-0.2in}
    % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \includegraphics[width=0.5\textwidth]{sec/images/qualitative_coco.pdf}
    %\vspace{-2em}
    \captionof{figure}{{\bf Qualitative Results} for 1-shot GFSS on COCO-20$^i$. The leftomost two columns show image and ground truth mask; (Third) Baseline without causal attention; (Fourth); Ours in inductive setting; (Fifth) Ours in transductive setting; (Last) DIaM~\cite{hajimiri2023strong}. \leon{Last row illustrates a {\em failure}.} }
    \label{fig:qual_supp}
\vspace{-8pt}
\end{figure}

\paragraph{Class-wise Results.} 

In Table~\ref{tab:classwise}, we present the base mIoU and novel mIoU, calculated as the mean across all base and novel classes, respectively. The overall mean mIoU of the Generalized Few-Shot Segmentation (GFSS) is determined by averaging these values, in accordance with the evaluation protocol outlined in~\cite{hajimiri2023strong}. Table~\ref{tab:classwise} provides insights into the 1-shot performance of our model within an inductive setting for each class (both base and novel) on the PASCAL-5$^i$ dataset, covering all four splits.

To emphasize the significance of our model's novel-to-base causal attention, we conduct a comparative analysis against the baseline without causal attention. The results, as depicted in the table, underscore a notable enhancement in performance for both novel and base classes across the various splits. Notably, on split-1, our base class performance exhibits a substantial improvement across most base classes.



% ----------------------------
\section{Multi-scale Analysis} 
\label{sec:multi-scale}
One of the key components of our approach involves prompting at multiple scales of the image. Our hypothesis posits that this strategy contributes to improved segmentation accuracy across objects of varying sizes. To substantiate this claim, Table~\ref{tab:object_size} presents an analysis of our model's performance in a transductive setting, evaluating objects of different sizes across various splits of Pascal-$5^i$, and comparing it with the transductive DIaM~\cite{hajimiri2023strong}. We categorize objects into three size categories: \emph{small}, \emph{medium}, and \emph{large}, based on the proportion of the image each object occupies. Specifically, we classify objects that occupy more than 30\% of the image as \emph{large}, those occupying between 10-30\% as \emph{medium}, and the remainder as \emph{small}. As depicted in the table, our approach consistently outperforms transductive DIaM~\cite{hajimiri2023strong} across objects of all sizes, notably excelling on small-sized objects.

\section{Additional Qualitative Results}
\label{sec:add-qual}
In Figure 5 of the main manuscript, we presented the qualitative results for 1-shot Generalized Few-Shot Segmentation (GFSS) using our model on PASCAL-5$^i$ in both inductive and transductive settings. We compared our outcomes against the baseline lacking causal attention and transductive DIAM~\cite{hajimiri2023strong}. However, no results were shown for COCO-20$^i$. Therefore, in Figure~\ref{fig:qual_supp}, a similar qualitative analysis is presented for 1-shot GFSS on COCO-20$^i$.

As observed, in the first image, the baseline without novel-to-base causal attention fails to appropriately segment the novel class \emph{bus}. The model with causal attention can segment the \emph{bus} with higher accuracy, further improved by transduction. In comparison, the segmentation quality of \emph{bus} in transductive DIAM~\cite{hajimiri2023strong} is considerably worse. In the second image, the baseline without causal attention can detect the novel category \emph{toilet} but misclassifies \emph{sink} and other unlabeled pixels (the tub) as a \emph{toilet}. Adding novel-to-base attention slightly improves segmentation quality but is still unable to correctly classify the \emph{sink}. However, adding transduction loss helps our model correctly classify it. Although DIAM can correctly classify \emph{sink}, it mostly misses the novel category \emph{toilet}. Similarly, in the third image, DIAM completely misses novel classes \emph{orange} and \emph{cup}. Our baseline without causal attention can identify both but with poor accuracy. Our model in the inductive setting can segment both the novel classes \emph{orange} and \emph{cup} with a higher degree of accuracy. Our model in the transductive setting, however, performs worse as it misses \emph{cup}. In the fourth image, both DIAM and the baseline without causal attention miss the novel class \emph{pizza}, and base classes \emph{broccoli} and \emph{oven}. Our models in both inductive and transductive settings can segment \emph{pizza} but fail to identify \emph{broccoli} and \emph{oven}. The fifth image showcases the importance and strength of multi-scale prompting. All our models can detect the small object \emph{baseball gloves} (base class) which DIAM misses. Moreover, DIAM performs worse in segmenting the base class \emph{baseball bat}. Similarly, DIAM and the baseline without causal attention miss novel classes \emph{surfingboard} and \emph{horse} completely in the sixth and seventh images, respectively. Our models (in inductive and transductive settings) can correctly segment them with good accuracy. However, in the seventh image, all methods fail to identify the novel class \emph{book}. Finally, we show a case where DIAM outperforms us in correctly segmenting the novel category \emph{frisbee}. Our models (inductive and transductive) incorrectly classify \emph{frisbee} as \emph{kite}.

Overall, these qualitative results demonstrate the strong performance of our model on both base and novel classes in both inductive and transductive settings. They also underscore the importance of the novel-to-base causal attention module and the multi-scale prompting approach.

%------------------------
\section{Societal Impact}
\label{sec:societal}
Few-shot object segmentation has multiple positive societal impacts as it can be used for a variety of useful applications, \eg, robot manipulation, augmented/virtual reality and assistive technologies (\eg, aid to the blind and low-level vision)~\cite{massiceti2021orbit}. 
% The ability to identify and segment objects guided by few examples can be used in such application areas. 
It can also help in democratizing computer vision research by  enabling low resourced communities to use the technology, \eg, Africa to develop their own techniques with the limited labelled data available.

However, as with many AI abilities, few-shot object segmentation also can have negative societal impacts. 
Nonetheless, we strongly believe these misuses are available in both few-shot and non few-shot methods and are not tied to the specific few-shot case. On the contrary, we argue that empowering developing countries towards decolonizing artificial intelligence is critical towards a decentralized and ethical AI approach.

%\eg through application to target tracking in military systems. To some extent, movements are emerging to limit such applications, \eg  pledges on the part of researchers to ban use  of artificial intelligence in weaponry systems. We have participated in signing that pledge and are supporters of its enforcement through international laws. 




